Complementing Lexical Retrieval with Semantic Residual Embedding

This paper presents CLEAR, a retrieval model that seeks to complement classical lexical exact-match models such as BM25 with semantic matching signals from a neural embedding matching model. CLEAR explicitly trains the neural embedding to encode language structures and semantics that lexical retrieval fails to capture with a novel residual-based embedding learning method. Empirical evaluations demonstrate the advantages of CLEAR over state-of-the-art retrieval models, and that it can substantially improve the end-to-end accuracy and efficiency of reranking pipelines.

==> sections/060experiments-covid.tex <==
\section{Zero-shot adaptation to TREC-COVID}
We analyze the performance of \CLEAR on the CORD-19 dataset \citep{Wang2020CORD19TC} (TREC-COVID ad-hoc search challenge\footnote{\url{https://ir.nist.gov/covidSubmit/index.html}}) to test its performance under a \emph{zero-shot, cross-domain} ad hoc retrieval scenario with zero training data. CORD-19 contains scientific articles related to the recent COVID-19 pandemic.  An effective retrieval system can help researchers, clinicians, and policymakers to understand the virus and combat the pandemic. However, state-of-the-art neural models may face challenges of lacking training data.  %Old lexical retrieval models, although does not require training, have only limited ability to understand the meanings behind the queries and the documents. 

We follow the settings of TREC-COVID's Round 2. The document set is the 5/1/2020 version of CORD-19, roughly containing 60k articles related to COVID-19. We use the Round 2 relevance judgments for evaluation, the query set of which contains 35 queries. Similar to TREC2019 DL queries, these queries are judged by NIST assessors with multiple relevant documents and graded labels. No training set is available. 

\paragraph{Zero-Shot Adaptation} %We used several simple techniques to develop a \CLEAR model for TREC-COVID without training the model on TREC-COVID queries and labels. 
We follow \citet{macavaney2020sledge} and initialize \CLEAR with SciBERT \citep{beltagy2019scibert} instead of BERT. Additionally, we fine-tune the masked language model of SciBERT on the CORD-19 documents for 10 epochs, to pick up COVID-19 specific vocabularies. \CLEAR is trained with $160$k examples from the MS MARCO passage ranking dataset. 
%For the lexical retrieval side of \CLEAR, training used the BM25 retrieval on MS MARCO; 
Lexical retrieval during inference adopted the Anserini BM25 fusion results using multiple document fields, which show stronger performance than the original BM25 on TREC-COVID\footnote{~Document contain 3 fields: title, abstract, and body. The fusion method computes BM25 on these fields respectively and fuses under equal weights. Detailed information can be found at~\url{https://ir.nist.gov/covidSubmit/archive/round2/r2.fusion2.pdf}}. For the neural embedding part, only the title and abstract are used due to their brevity; the two fields are concatenated and encoded into a single vector. The trained \CLEAR is used on TREC-COVID \emph{without any in-domain gradient update}.

\paragraph{Baselines} We include the following baselines for analysis: \textbf{BM25 (fusion)}, which is the same BM25 with multi-field fusion method as in the lexical part of \CLEAR; \textbf{ZS Neural only}, a pure neural embedding retriever using the same zero-shot adaptation settings as \CLEAR; and the \emph{best automatic run}\footnote{~Non-automatic runs modified queries or models using relevance feedback from the previous run or with manual modification, hence are not included for comparison. Information can be found at \url{https://ir.nist.gov/covidSubmit/archive/archive-round2.html}.} submitted to TREC-COVID Round 2. The run is named \textbf{GUIR-S2-run1} which used BM25 initial retrieval, SciBERT reranking, pseudo-relevance feedback, and a fusion of these rankings to further improve the accuracy.\footnote{Detailed information for GUIR-S2-run1 can be found at \url{https://ir.nist.gov/covidSubmit/archive/round2/GUIR\_S2\_run1.pdf}}
\begin{table}[t]
\centering

\adjustbox{max width=\linewidth}{
\begin{tabular}{llll}
\toprule
Model &  P@5    &  NDCG@10 &  R@1k  \\\midrule 
{\small $1$} BM25 (fusion)          & 0.680$^{2}$ & 0.555$^{2}$  & 0.647$^{2}$      \\
%anserini.r2.fusion2   & 0.555 & & 0.663 \\ \hline 
{\small $2$} ZS Neural only  & 0.468 & 0.371  & 0.553      \\ \midrule
{\small $3$} ZS \CLEAR        & \textbf{0.760}$^{12}$ & \textbf{0.636}$^{124}$  &  \textbf{0.716}$^{124}$     \\ \midrule 
{\small $4$} GUIR-S2-run1  & 0.749$^{12}$ & 0.625$^{12}$  & 0.660$^{12}$      \\ 
\bottomrule
%CLEAR+BERT-Reranker  & 0.676 & 0.601  & 0.649      \\\hline \hline
\end{tabular}}
\caption{Zero-shot results on TREC-COVID Round 2. Again, superscripts 1--4 indicate statistically significant improvements over the corresponding methods.} %All models are trained on a subset of the MS MARCO training set without any in-domain fine-tuning on TREC-COVID.}
\label{tab:covid}
\end{table}

\paragraph{Results} Results are shown in Table~\ref{tab:covid}. Zero-Shot \CLEAR substantially outperforms BM25 (fusion), demonstrating that the semantic patterns learned by \CLEAR are transferable, and can complement the lexical retrieval under an out-of-domain scenario. On the other hand, zero-shot neural-only retriever is significantly worse than BM25, indicating that embeddings alone are less transferable to other domains. Notably, zero-shot \CLEAR outperforms GUIR-S2-run1, the best automatic run that uses a computation-expensive BERT reranker and pseudo-relevance feedback procedures.  In contrast, \CLEAR only performed a single round of retrieval without reranking. These results demonstrate the generalizability of \CLEAR under low-resource, cross-domain settings, showing promise for rapidly building effective and efficient retrieval systems for new domains with limited training data.


==> sections/table1.bak.tex <==

\begin{table*}[t]
\centering
\adjustbox{max width=\linewidth}{
\begin{tabular}{lcccccc}
\toprule
 \multirow{2}{*}{Model}              & \multicolumn{2}{c}{MS MARCO Dev}                       & \multicolumn{4}{c}{TREC2019 DL}                                                                                                                                    \\ \cmidrule(lr){2-3} \cmidrule(lr){4-7}
                  & \small MRR@10   & \small R@1k & \small MRR   & \small NDCG@10 & \small MAP@1k & \small R@1k \\ 
                  \midrule
 BM25                & 0.191 & 0.864                                                 & 0.825 & 0.506                                              & 0.377                                               & 0.738                                                 \\
BM25+RM3            &   0.166    &     0.861                                                & 0.818 & 0.555                                             & 0.452                                               & 0.789                                                 \\
DeepCT              & 0.243 & 0.913                                                 & 0.858 & 0.551                                              & 0.422                                               & 0.756                                                 \\
DeepCT+RM3          &  0.232     & 0.914                                                        & 0.924 & 0.601                                              & 0.481                                               & 0.794                                                 \\ \midrule
Neural only            & 0.308 & 0.928                                                 & 0.842 & 0.594                                              & 0.307                                               & 0.584                                                 \\ \midrule
\CLEAR               & \textbf{0.338} & \textbf{0.969}                                                 & \textbf{0.979} & \textbf{0.699}                                              & \textbf{0.511}                                               & \textbf{0.812}                                                  \\
~$-$ Error-based Sampling $\Rightarrow$ Random &    \ssl{0.241}    & \ssl{0.926}  &   \ssl{0.850}    &   \ssl{0.553}   & \ssl{0.409}    & \ssl{0.779}   \\ 
~$-$ Residual Margin $\Rightarrow$ Constant Margin       & \ssl{0.314} & \ssl{0.955}                                            & 0.928 & \ssl{0.664} & \ssl{0.455}                                         & 0.794 \\ \bottomrule
\end{tabular}}
